On the Efficiency of the Walrasian Mechanism

Central results in economics guarantee the existence of efficient equilibria for various classes of markets. An underlying assumption in early work is that agents are price-takers, i.e., agents honestly report their true demand in response to prices. A line of research in economics, initiated by Hurwicz (1972), is devoted to understanding how such markets perform when agents are strategic about their demands. This is captured by the \emph{Walrasian Mechanism} that proceeds by collecting reported demands, finding clearing prices in the \emph{reported} market via an ascending price t\^{a}tonnement procedure, and returns the resulting allocation. Similar mechanisms are used, for example, in the daily opening of the New York Stock Exchange and the call market for copper and gold in London. In practice, it is commonly observed that agents in such markets reduce their demand leading to behaviors resembling bargaining and to inefficient outcomes. We ask how inefficient the equilibria can be. Our main result is that the welfare of every pure Nash equilibrium of the Walrasian mechanism is at least one quarter of the optimal welfare, when players have gross substitute valuations and do not overbid. Previous analysis of the Walrasian mechanism have resorted to large market assumptions to show convergence to efficiency in the limit. Our result shows that approximate efficiency is guaranteed regardless of the size of the market.

==> tatonnement-extensions.tex <==
\section{Extensions to Bayesian settings via smoothness}

In this section we use the smooth auctions framework of Syrgkanis and Tardos \cite{Syrgkanis13} to
extend our result to Bayesian settings. In this setting, each
agents value $v_i$ is drawn independently from a distribution $F_i$ over gross substitute
valuation functions. Nothing is assumed about the distribution except independence across agents.
Each agent $i$ knows the realization of his value $v_i$ but only the distributions over other
agents values. His strategy is a (possibly randomized) mapping between his value $v_i$ and
declared value, which we denote by $b_i(v_i)$. We say that the vector of mappings
$\vc{b} = (b_1, \hdots, b_n)$ is a Bayes Nash equilibrium if:
$$\E_{\vc{v}} \E_{\vc{b}} [u_i(b_i, \vc{b}_{-i}) \vert v_i] \geq
 \E_{\vc{v}} \E_{\vc{b}} [u_i(b'_i, \vc{b}_{-i}) \vert v_i], \quad \forall i \in [n], v_i \in \text{supp}(F_i)  $$

Syrgkanis and Tardos \cite{syrgkanis} define the concept of smooth mechanisms based on Roughgarden's smoothness framework \cite{Roughgarden09, Roughgarden12} as follows:

\begin{defn}[smooth mechanisms]\label{dfn:smooth_mechanisms}
Given a vector of valuations $\vc{v}$ and a vector of bids $\vc{b}$, let $\textsc{Opt}(\vc{v})$ be the value of the optimal allocation according to $\vc{v}$ and $\textsc{SW}(\vc{v},\vc{b})$ be the welfare of the equilibrium induced by bids $\vc{b}$ on agents with values $\vc{v}$.
A mechanism is $(\lambda, \mu)$-smooth if for each agent there is a deviating bid $s_i(b_i, \vc{v})$ such that: $\sum_i u_i(s_i(b_i, \vc{v}), \vc{b}_{-i}) \geq \lambda \cdot \textsc{Opt}(\vc{v}) - \mu \cdot \textsc{SW}(\vc{v},\vc{b}) $.
\end{defn}

Their main result is that:

\begin{theorem}[Syrgkanis and Tardos \cite{syrgkanis}]
If a mechanism is $(\lambda, \mu)$-smooth, then its Bayes Nash Price of Anarchy is bounded by $\frac{\lambda}{1+\mu}$, i.e., for any Bayes Nash equilibrium, $\E_\vc{v} \E_{\vc{b}} \sum_i [v_i(X_i(\vc{b}))] \geq \frac{\lambda}{1+\mu} \cdot \E_\vc{v} [ \sum_i v_i(X_i(\vc{v})) ]$.
\end{theorem}

The same bound on the Price of Anarchy holds for coarse-correlated equilibria, which capture both mixed Nash equilibria and the outcome of no-regret learning strategies. A crucial fact in Definition \ref{dfn:smooth_mechanisms} that enables the bound on the Bayes-Nash Price of Anarchy is that the deviation depends only on the values of other agents \emph{but not on their bids}. Now, we argue that this is the case in our proof:

\begin{lemma}
The Walrasian Mechanism is $(\frac{1}{2}, 1)$-smooth.
\end{lemma}

We note that our proof follows considering the set $X_i^*$ each player $i$ would receive in the optimal allocation and sampling a random subset $S \sim \mathcal{H}[X_i^*]$ of size $\frac{1}{2}\abs{X_i^*}$ and then considering a deviation to a bid $b'_i(T) = v_i(S \cup T)$. We note that the deviating bid used the valuations of other agents in order to compute  $X_i^*$ but didn't use the bids of other agents in order to compute the deviation.

\section{Efficiency of the VCG Mechanism}

In Example \ref{example:2_bound_unit_demand}, we saw an example of a non-overbidding equilibrium of the VCG mechanism (which coincides with the Walrasian mechanism for unit-demand agents) with an inefficient outcome. Here we show that if we assume non-overbidding instead of the usual stronger assumption that player will employ the truthtelling best-response, we get a bound of $2$ for the Price of Anarchy of VCG.

In what follows, the VCG mechanism is the mechanism that proceeds by collecting reported valuations $b_i$, and allocated according to the optimal allocation $X_i(\vc{b})$ for the reported bids. Each agent $i$ is charged payment $\pi_i = W^{\vc{b}_{-i}}(X_i(\vc{b}) \vert \overline{X_i(\vc{b})})$.


\begin{lemma}
Given a valuation profile of gross substitute valuations, then for any $\gamma$-bounded overbidding equilibrium the Price of Anarchy is bounded by $1+\gamma$. In particular, it is bounded by $2$ for non-overbidding players.
\end{lemma}

\begin{proof}
Let $X_i(\vc{b})$ be the allocation of agent $i$ in equilibrium and let $X_i^*$ be his optimal allocation. Then:
$$\begin{aligned} u_i(\vc{b}) & \geq u_i(v_i, \vc{b}_{-i}) = v_i(X_i(v_i, \vc{b}_{-i})) - [W^{\vc{b}_{-i}}([m]) - W^{\vc{b}_{-i}}(\overline{X_i(v_i, \vc{b}_{-i})})] \geq \\ & \geq v_i(X_i^*) + W^{\vc{b}_{-i}}(\overline{X_i^*}) - W^{\vc{b}_{-i}}([m]) =  v_i(X_i^*) + W^{\vc{b}_{-i}}(X_i^*  \vert \overline{X_i^*}) \end{aligned} $$
Now, one can use the same argument as in the proof of Theorem \ref{thm:pure_poa} to argue that $W^{\vc{b}_{-i}}(X_i^*  \vert \overline{X_i^*}) \leq \sum_i b_i(X_i(\vc{b}))$. Notice that this argument requires $b_i$ to be gross substitutes so that we can use the submodularity of the $W^{\vc{b}}(S)$ function. Summing over all $i$ and using that $\sum_i u_i(\vc{b}) \leq \sum_i v_i(X_i(\vc{b}))$ and $\sum_i b_i(X_i(\vc{b})) \leq \gamma \cdot \sum_i v_i(X_i(\vc{b}))$, we get the desired result.
\end{proof}

\section{Dutch Walrasian Mechanism}

So far, we considered the version of the Walrasian mechanism that implements the lowest price vector in the lattice. This is the mechanism the Gul and Stachetti \cite{GulStachetti00} call the \emph{English Auction for Differentiated Commodities}, since its outcome is a product an ascending process that much resembles an English Auction. Analogously, one could define a \emph{Dutch Auction for Differentiated Commodities}, which would be the allocation one would achieve by a descending price procedure. We will define here the Dutch auction as being the auction that allocates according to a Walrasian equilibrium using the higher price vector in the lattice. For a single item auction, it would correspond to the first price auction.

The Dutch Walrasian Mechanism will collect bids and allocate the set $X_i(\vc{b})$ as the English Walrasian Mechanism but will charge payments $\sum_{j \in X_i(\vc{b})} W^{\vc{b}}(j \vert [m] \setminus j)$, which is the price vector in the highest point of the lattice (Lemma \ref{lemma:shadow_prices}). Our main result is a bound of $8$ on the Price of Anarchy that holds \emph{independent of non-overbidding assumptions}.

\begin{theorem}\label{thm:dutch}
Given a valuation profile $\vc{v}$ composed of gross substitute valuations and a bid profile $\vc{b} \in \nash(\vc{v})$ , then $\sum_i v_i(X_i(\vc{b})) \geq \frac{1}{8} \cdot \sum_i v_i(X_i(\vc{v}))$. In other words, the Price of Anarchy is bounded by $8$.
\end{theorem}

\begin{proof}
Let $\vc{b}$ be a Nash equilibrium and let $(X_i^*, \hdots, X_n^*)$ be the optimal allocation. We assume without loss of generality that $\abs{X_i^*}$ is even. Now, consider the deviation where each player $i$
\end{proof}


==> tatonnement-generic-xos.tex <==
\section{Generic Mechanisms for XOS bidders}

Consider a set $[m]$ of items and $n$ agents with valuations over such
items. It will be convenient to represent a bundle $S \subseteq [m]$ by the indicator vector $\vc{x} \in \{0,1\}^m$. Also, we will assume that valuations are XOS, i.e., they can be written as: $v_i(\vc{x}) = \max_{t \in \mathcal{T}_i} \vc{w}_{it} \cdot \vc{x}$, where   $\vc{w}_{i}^t \in \R^m_+$ is a vector of weights. Also, given a vector of valuation functions $\vc{v} = (v_1, v_2, \hdots, v_k)$, we will define the welfare function $W^{\vc{v}} : \Z^m \rightarrow \R_+$ such that:
$$W^{\vc{v}}(\vc{x}) = \max \{ \textstyle\sum_{i=1}^k v_i(\vc{x}_i) ; \textstyle\sum_{i=1}^k \vc{x}_i \leq \vc{x} \} $$
Whenever $v_1, \hdots, v_k$ are XOS functions, then $W^{\vc{v}}$ is also in XOS.

Consider any mechanism that elicits XOS valuations, collecting reports $b_1, \hdots, b_n$ and outputs the optimal allocation of the goods under such declarations and charges some payment $\pi_i(\vc{b})$ that is at most the value of the set allocated to the agent, i.e., $\pi_i(\vc{b})  \leq b_i(\vc{x}_i(\vc{b}))$. Some family of mechanisms that allocate according to such rules are:
\begin{itemize}
\item VCG mechanism: $\pi_i = W^{\vc{b}_{-i}}(\vc{x}_i \vert \vc{x}_{-i} )$.
\item English Walrasian mechanism: $\pi_i = \sum_{j \in \vc{x}_i} W^{\vc{b}}( \vc{e}_j \vert \one )$.
\item Dutch Walrasian mechanism: $\pi_i = \sum_{j \in \vc{x}_i} W^{\vc{b}}( \vc{e}_j \vert \one -  \vc{e}_j )$.
\item First price mechanism: $\pi_i = b_i(\vc{x}_i)$.
\end{itemize}

We note that all mechanisms above have the same allocations and increasing payments, in the sense that:
$$W^{\vc{b}_{-i}}(\vc{x}_i \vert \vc{x}_{-i} ) \leq \sum_{j \in \vc{x}_i} W^{\vc{b}}( \vc{e}_j \vert \one ) \leq \sum_{j \in \vc{x}_i} W^{\vc{b}}( \vc{e}_j \vert \one -  \vc{e}_j ) \leq  b_i(\vc{x}_i)$$
Actually, this ranking is true for gross substitutes $\vc{b}$. For XOS valuations, the ranking might not be true. Consider the following  example adapted from Example 5 in Lehmann, Lehmann and Nisan. Consider three players $1,2,3$ and three items $A,B,C$. Let the valuations be:
$$v_1(\vc{x}) = 100 (x_A + x_B) \qquad v_2(\vc{x}) = x_1 + 2 x_2 \qquad v_3(\vc{x}) = \min\{6, 3 x_A + 5 x_B + 3 x_C \}$$
Now, the payment of player $1$ under VCG is $3$. Under the English Walrasian mechanism, however, it is $2$. Notice that for those examples, the valuations are even submodular, but not gross substitutes. For gross substitutes, it follows easily using the submodularity of the $W^{\vc{b}}$ function:
$$W^{\vc{b}}(\vc{e}_j \vert \one) \geq W^{\vc{b}}(\vc{x}_j \vert \one) \geq [b_i(\vc{x}_i) + W^{\vc{b}_{-i}}(\one)] - [b_i(\vc{x}_i) + W^{\vc{b}_{-i}}(\vc{x}_{-i})] = W^{\vc{b}_{-i}}(\vc{x}_{i} \vert \vc{x}_{-i})$$
and the last one follows from:
$$\begin{aligned}\sum_{j \in \vc{x}_i} W^{\vc{b}}( \vc{e}_j \vert \one -  \vc{e}_j ) & \leq \sum_{j \in \vc{x}_i} W^{\vc{b}} [b_i(\vc{x}_i) + W^{\vc{b}_{-i}}(\one - \vc{x}_i)] - [b_i(\vc{x}_i - \vc{e}_j) + W^{\vc{b}_{-i}}(\one - \vc{x}_i)]   = \\ & = \sum_{j \in \vc{x}_i} b_i(\vc{e}_j \vert \vc{x}_i - \vc{e}_j) \leq b_i(\vc{x}_i) \end{aligned}$$

\vspace{1cm}

Now, consider any such mechanism and consider a deviation for player $i$ to declare $\frac{1}{2}  v_i$. Let $\vc{x}'_i$ be his allocation under $(\frac{1}{2} v_i, \vc{b}_{-i})$, then:
$$u_i(\vc{b}) \geq u_i(v_i, \vc{b_{-i}}) =  v_i(\vc{x}'_i) - \pi_i(v_i, \vc{b_{-i}}) \geq  v_i(\vc{x}'_i) - \frac{1}{2}  v_i(\vc{x}'_i) = v_i(\vc{x}'_i)$$
by the allocation rule, it is the case that:
$$\frac{1}{2} v_i(\vc{x}'_i) + W^{\vc{b}_{-i}}(\one - \vc{x}'_i) \geq \frac{1}{2} v_i(\vc{x}^*_i) + W^{\vc{b}_{-i}}(\one - \vc{x}^*_i)$$
where $(\vc{x}^*_1, \hdots, \vc{x}^*_n)$ is the allocation that optimizes $\sum_i v_i(\vc{x}_i^*)$. Therefore, we have:
$$u_i(\vc{b}) \geq  \frac{1}{2} v_i(\vc{x}^*_i) + W^{\vc{b}_{-i}}(\one - \vc{x}^*_i) - W^{\vc{b}_{-i}}(\one - \vc{x}'_i) \geq \frac{1}{2} v_i(\vc{x}^*_i) -  W^{\vc{b}_{-i}}(\vc{x}^*_i \vert \one - \vc{x}^*_i)$$

Now, we sum for all $i$ and bound each term separately. Notice that $u_i(\vc{b}) \leq v_i(\vc{x}_i)$. As for the  $W^{\vc{b}_{-i}}(\vc{x}^*_i \vert \one - \vc{x}^*_i)$ term, we would like to prove that  $\sum_i W^{\vc{b}_{-i}}(\vc{x}^*_i \vert \one - \vc{x}^*_i) \leq c\cdot \sum_i b_i(\vc{x}_i)$ for some constant $c$. Since bids are XOS, then there is $\vc{w}_i$ such that $b_i(\vc{x}_i) = \vc{w}_i \cdot \vc{x}_i$, then $W^{\vc{b}}(\one) = \sum_i \vc{w}_i \cdot \vc{x}_i$. We know that:
$$\sum_i  W^{\vc{b}_{-i}}(\vc{x}^*_i \vert \one - \vc{x}^*_i) = \sum_i W^{\vc{b}_{-i}}(\one) - W^{\vc{b}_{-i}}(\one - \vc{x}_i^*) \leq \sum_i \left[ W^{\vc{b}}(\one) - \sum_{j \neq i} b_j (\vc{x_j} \cap \one - \vc{x}_i^*) \right]$$
since one possible allocation of $\one - \vc{x}_i^*$ to $\vc{b}_{-i}$ is simply to project the optimal allocation. Now we know that: 
$$ \sum_i \sum_{j \neq i} b_j (\vc{x_j} \cap \one - \vc{x}_i^*)  \geq \sum_i \sum_{j \neq i} \vc{w}_j \cdot (\vc{x_j} \cap \one - \vc{x}_i^*) \geq (n-2) \sum_i \vc{w}_j \cdot \vc{x}_j = (n-2) \cdot W^{\vc{b}}(\one)$$ 
Putting everything together, we get: $\sum_i W^{\vc{b}_{-i}}(\vc{x}^*_i \vert \one - \vc{x}^*_i) \leq 2 \cdot \sum_i b_i(\vc{x}_i)$. This implies in the end that:
$$2 \cdot \sum_i b_i(\vc{x}_i) + \sum_i v_i(\vc{x}_i) \geq \frac{1}{2} \sum_i v_i(\vc{x}_i^* ) $$
under a $\gamma$-no-overbidding assumption, we get: $2(1+2\gamma)$ Price of Anarchy. For the case where agents need to report gross substitute valuations, we get $2(1+\gamma)$, using the following: let $(\vc{y}_i,\vc{y}_{-i})$ be the allocation to $i$ and $-i$ of $\one - \vc{x}_i^*$, then:
$$\begin{aligned}W^{\vc{b}}(\vc{x}_i^* \vert \one - \vc{x}_i^* ) & = W^{\vc{b}}(\one) - W^{\vc{b}}( \one - \vc{x}_i^* ) \geq [b_i(\vc{y}_i) + W^{\vc{b}_{-i}}(\vc{y}_{-i} + \vc{x}_i^*)] - [b_i(\vc{y}_i) + W^{\vc{b}_{-i}}(\vc{y}_{-i})] =\\ & = W^{\vc{b}_{-i}}(\vc{x}_i^* \vert \vc{y}_{-i}) \geq W^{\vc{b}_{-i}}(\vc{x}_i^* \vert \one - \vc{x}_i^*)\end{aligned}$$
where the last step follows from the submodularity of $W^{\vc{b}}$. Now, we can use that:
$$\sum_i W^{\vc{b}_{-i}}(\vc{x}_i^* \vert \one - \vc{x}_i^*) \leq \sum_i W^{\vc{b}}(\vc{x}_i^* \vert \one - \vc{x}_i^* ) \leq \sum_i W^{\vc{b}}(\vc{x}_i^* \vert \sum_{j<i} \vc{x}_j^* ) = W^{\vc{b}}(\one) = \sum_i b_i(\vc{x}_i)$$

\section{Questions}

\begin{itemize}
\item under which conditions can one guarantee no-overbidding ? besides of course first price and the VCG payment rule ? for the English Walrasian we can show that overbidding can be profitable ? is this also true for the Dutch Walrasian mechanism ? also, maybe we can show that overbidding by more then twice the value might be dominated or something like that.
    
\item for the English Walrasian auction, we have a lower bound of $2$ and an upper bound of $4$ for no-overbidding equilibria. can we close this gap by giving a better upper bound ?
    
\item approximate welfare maximization. if the mechanism selects an allocation that is a $c$-approximation rather then the exact solution,

\end{itemize}
